SoFaiR: Single Shot Fair Representation Learning

To avoid discriminatory uses of their data, organizations can learn to map them into a representation that filters out information related to sensitive attributes. However, all existing methods in fair representation learning generate a fairness-information trade-off. To achieve different points on the fairness-information plane, one must train different models. In this paper, we first demonstrate that fairness-information trade-offs are fully characterized by rate-distortion trade-offs. Then, we use this key result and propose SoFaiR, a single shot fair representation learning method that generates with one trained model many points on the fairness-information plane. Besides its computational saving, our single-shot approach is, to the extent of our knowledge, the first fair representation learning method that explains what information is affected by changes in the fairness / distortion properties of the representation. Empirically, we find on three datasets that SoFaiR achieves similar fairness-information trade-offs as its multi-shot counterparts.

==> experiment_app.tex <==
\section{Experimental Protocol}

\subsection{DSprites-Unfair}
We adapt DSprites\footnote{\url{https://github.com/deepmind/dsprites-dataset/}} to our fairness problem. DSprites (\cite{dsprites17}) contains $64$ by $64$ black and white images of various shapes (heart, square, circle), that are constructed from six independent factors of variation: color (black or white); shape (square, heart, ellipse), scales (6 values), orientation (40 angles in $[0, 2\pi]$); x- and y- positions (32 values each). The dataset results in $700K$ unique combinations of factor of variations. We modify the sampling to generate a source of potential unfairness. The sensitive attribute encodes which quadrant of the circle the orientation angle belongs to: $[0, \pi/2]$, $[\pi/2, \pi]$, $[\pi, 3/2\pi]$ and $[3/2\pi, 2\pi]$. All factors of variation but shapes are uniformly drawn. When sampling shapes, we assign to each possible combination of attributes a weight proportional to $1 + 10 \left[\left(\frac{i_{orientation}}{40})\right)^{3} + \left(\frac{i_{shape}}{3}\right)^{3}\right]$ , where $i_{shape}\in \{0, 1, 2\}$ and $i_{orientation}=\{0, 1, ..., 39\}$. This weight scheme generates a correlation between shapes and sensitive attributes (orientation).
%Since shapes and orientation are correlated, a downstream task predicting shapes could risk to discriminate against some orientation. 

\subsection{Adults / Heritage}
The \textbf{Adults} dataset \footnote{https://archive.ics.uci.edu/ml/datasets/adult}  contains $49K$ individuals with information to professional occupation, education attainment, capital gains, hours worked, race and marital status. We consider two variants of the Adults dataset: \textbf{Adults-Gender} and \textbf{Adults-Gender-Race}. In Adults-Gender we define as sensitive attributes the gender to which each individual self-identifies to.  In Adults-Gender-Race, we define as sensitive attribute an intersection of the gender and race an individual self-identifies to. For both Adults-Gender and Adults-Gender-Race, the downstream task label $Y$ correspond to whether individual income exceeds $50K$ per year.

The \textbf{Health Heritage} dataset \footnote{https://foreverdata.org/1015/index.html} contains $95K$ individuals with $65$ features related to clinical diagnoses and procedure, lab results, drug prescriptions and claims payment aggregated over $3$ years (2011-2013). We define as sensitive attributes a $18-$ dimensional variable that intersects the gender which individuals self-identify to and their reported age. 
The downstream task label $Y$ relates to whether an individual has a non-zero Charlson comorbidity Index, which is an indicator of a patient's 10-year survival rate.

\subsection{Comparative Methods}

\paragraph{LATFR:} This method ~\cite{madras2018learning} controls the mutual information $I(Z, S)$ via the cross-entropy of an adversary that predicts $S$ from $Z$. LATFR controls the fairness properties of the representation $Z$ with a single parameter in $\{ 0.1, 0.2, 0.3, 0.5, 0.7, 1.0, 1.5, 2.0, 3.0, 4.\}$ as prescribed in the original paper. 

\paragraph{Maxent-ARL:} This method \cite{roy2019mitigating} is a variant of LATFR that replaces the cross-entropy of the adversary with the entropy of is prediction. The fairness properties of $Z$ are controlled by a single parameter that we vary between $0$ and $1$ in steps of $0.1$, between $1$ and $10$ in steps of 1 and then between $10$ and $100$ in steps of 10.

\paragraph{$\beta-$VAE:}This method \cite{higgins2016beta,gitiaux2021fair} controls for $I(Z, S)$ by controlling the Kullback-Leibler divergence between $p(z)$ and an isotropic Gaussian prior. The fairness properties of the representations are controlled via the coefficient $\beta$ on the Kullback-Leibler divergence term: larger values of $\beta$ force $Z$ be more noisy, reduce the capacity of the channel between the data and the representation and thus, the mutual information $I(Z, X)$. We vary the value of $\beta$ between 0 and 1 in steps of 0.05.

\paragraph{CVIB:} This method ~\cite{moyer2018invariant} controls for $I(Z, S)$ via both the Kullback-Leibler divergence between $p(z)$ and an isotropic Gaussian prior (as in $\beta$-VAE) and an information-theory upper bound. The first term is controlled by a parameter $\beta$ that takes values in $\{0.001, 0.01, 0.1\}$; the second is controlled by a parameter $\lambda$ that vary between 0.01 to 0.1 in steps of 0.01 and 0.1 to 1.0 in steps of 0.1 (\cite{gupta2021controllable}).


\subsection{Architectures} 

\begin{table}[h]
    \centering
    \begin{tabular}{l|l|l|l|l}
    \toprule
    Dataset & Number of iterations & Learning rate \\
    \midrule
    DSprites & 546K &  $0.3 \times 10^{-4}$ \\
      \midrule
      Adults & 27K & $0.3 \times 10^{-4}$ \\
       \midrule
       Heritage & 74K & $0.3 \times 10^{-4}$ \\
       \bottomrule
\end{tabular}
\caption{Hyperparameter values for SoFaiR / MSFaiR.}
\label{tab: hyper}
\end{table}

\paragraph{Encoder-decoders.} For the DSprites dataset, the autoencoder architecture -- taken directly from \cite{creager2019flexibly} -- includes $4$ convolutional layers and $4$ deconvolutional layers and uses ReLU activations. For Adults and Heritage, the encoder and decoder are made of fully connected layers with ReLU activations. Table \ref{tab: arch} shows more architectural details for each dataset. Moreover, means $\mu$, scales $\gamma$ and mixture probabilities $\pi$ are modeled as fully connected linear layers with input dimension $1$ and output dimension d, i.e. the dimension of the latent space. We choose $K=5$ logistic distributions in the mixture. We also set the maximum number of bits per dimension, $A$, to be equal to 8. Other hyperparameter values are in Table \ref{tab: hyper}.

\paragraph{Auditor and task classifiers.} Downstream classifiers and fairness auditors are multi-layer perceptrons with $2$ hidden layers of $256$ neurons each. Learning rates for both auditing and downstream tasks are set to $0.001$

\subsection{Additional Details on Area under unfairness-distortion curves.} 
We compute the area under unfair-distortion curve, AUFDC, as follows: 
\begin{itemize}
\item Since we only generate a finite number of points, empirical fairness-distortion curves do not have to exhibit a perfectly decreasing and smooth behavior.Therefore, to compute our AUFDC metric,  we first filter out the points on the curve that have higher distortion than points with higher $I(Z, S)$. That is, for any point $(D, I)$, we remove all points $(D^{'}, I^{'})$ for which $D^{'}>D$ and $I^{'}>I$.
\item We estimate the largest obtainable mutual information $I_{max}$ between $Z$ and $S$ as
\begin{equation}
H(S) - \min_{c}E_{s, x}[-\log c(s|x)],
\end{equation}
where $c:\mathcal{X}\rightarrow \mathcal{S}$ are classifiers that predict $S$  from the data $X$. That is, we use an adversarial estimate of $I(X, S)$ and use this estimate as $I_{max}$, since by the data processing inequality ~\cite{cover2012elements}, $I(Z, S)\leq I(X, S)$. 
\item For models that do not reach $I(Z, S)=0$, we compute the distortion $D_{max}$ obtained by generating random representations; and then, we add to the AUFDC score, the area $I_{min} \times (D_{max} - D_{min})$ where  $(D_{min}, I_{min})$ is the point the furthest on the bottom right of the unfairness-distiortion curve achieved by the model.
\item To allow comparison across datasets, we normalize the value of AUFD by the area of the rectangle $[0, D_{max}]\times[0, I_{max}]$.
\end{itemize}

\subsection{Pareto Front Protocol}
To generate the Pareto fronts in Figure 4 of the main text and Figure 2 of the supplemental file, we implement the following protocol:
\begin{itemize}
    \item Train an encoder-decoder architecture and freeze its parameters;
    \item Train an auditing classifier $c:\mathcal{Z}\rightarrow \mathcal{S}$ to predict $S$ from $Z$;
    \item Train a downstream task classifier $T:\mathcal{Z}\rightarrow\mathcal{Y}$ to predict a task $Y$ from $Z$.
\end{itemize}
The encoder-decoder does not access the task labels during training and our representation learning framework remains unsupervised with respect to downstream task labels. 
%We split datasets into one training set used to train the encoder-decoder architecture; two test sets, one to train both task and auditing classifiers on samples not seen by the encoder-decoder; one to evaluate their performances. 

==> theorem1.tex <==
\section{Proof of Theorem 2.1}
First, we show the following identity: 
\begin{lem}
\label{lem: 1}
$I(Z,S)=I(Z, X) + H(X|Z, S) - H(X|S)$.
\end{lem} 

\begin{proof}
The proof of Lemma \ref{lem: 1} relies on multiple iterations of the chain rule for mutual information:
\begin{equation}\nonumber
\begin{split}
    I(Z, S) &\overset{(a)}{=} I(Z, \{X, S\}) - I(Z, X|S) \\
    & \overset{(b)}{=}I(Z, X) + I(Z, S|X)  - I(Z, X|S) \\
    & \overset{(c)}{=} I(Z, X)- I(Z, X|S) \\
    & \overset{(d)}{=}I(Z, X) - I(X, \{Z, S\}) + I(X, S) \\
    & \overset{(e)}{=}I(Z, X) - H(X) + H(X|Z, S) \\
    & + H(X) - H(X|S) \\
    & = I(Z, X) + H(X|Z, S) - H(X|S)
    \end{split}
\end{equation}
where $(a)$, $(b)$ and $(d)$ use the chain rule for mutual information; and, $(c)$ uses the fact that $Z$ is only encoded from $X$ and from $S$, so $H(Z|X, S)=H(Z|X)$ and $I(Z, S|X)=H(Z|X)-H(Z|X, S)=0$. And $(e)$ uses the fact that $I(X, S)=H(X) - H(X|S)$ and $I(X, \{Z, S\})=H(X) - H(X|Z, S)$. 
\end{proof}

Lemma \ref{lem: 1} implies that if the distortion is $d(X, \{Z, S\})=H(X|Z, S)$, the unfairness-distortion function is given by
\begin{equation}
\label{eq: chp5_frl_proof}
\begin{split}
I(D)= &\min_{f}I(Z, X) + H(X|Z, S) - H(X|S) \\
& \mbox{ s.t. } H(X, \{Z, S\}) \leq D \\
\end{split}
\end{equation}


Second, a fundamental theorem in rate-distortion shows that if the distortion is $d(X, \{Z, S\})=H(X|Z, S)$ the rate-distortion function is given by 
\begin{equation}
\label{eq: ib_proof}
R(D)=\min_{f} I(X, Z) \mbox{ s.t } H(X|Z, S) \leq D,
\end{equation}
and that $R(D)$ is a non-increasing convex function. The next Lemma shows how solution of the minimization problem \eqref{eq: ib_proof} solves the minimization problem \eqref{eq: chp5_frl_proof} whenever $\frac{\partial R(D)}{\partial D}\leq -1$


\begin{lem}
\label{lem: 2}
Let $D\geq 0$ be a distortion value. Assume that $\frac{\partial R(D)}{\partial D}\leq -1$. A solution $f^{*}$ of the minimization \eqref{eq: ib_proof} for $D$ is also solution of \eqref{eq: chp5_frl_proof}.
\end{lem}

\begin{proof}
At the optimum, the constraint in \eqref{eq: ib_proof} is binding and thus, that $H_{f^{*}}(X|Z, S)=D$, where the subs-script $f^{*}$ reminds that the code $Z$ depends on $f^{*}$. Consider now a solution $g^{*}$ of the minimization  \eqref{eq: chp5_frl_proof} for a distortion $D$. We consider two cases: case (I) the constraint is binding for $g^{*}$ in \eqref{eq: chp5_frl_proof}; case (II) the constraint is not binding for $g^{*}$ in \eqref{eq: chp5_frl_proof}. 


\textbf{case (I)}: $H_{g^{*}}(X|Z, S)=D$ and we have
\begin{equation}
\begin{split}
I(D) &= I_{g^{*}}(Z, X) + H_{g^{*}}(X|Z, S) - H(X|S)\\
     & = I_{g^{*}}(Z, X) + D -H(X|S) \\
     & \overset{(a)} {\geq} I_{f^{*}}(Z, X) + D -H(X|S), \\
     \end{split}
\end{equation}
where $(a)$ uses the fact that $f^{*}$ is solution of  \eqref{eq: ib_proof} and that $H_{g^{*}}(X|Z, S)\leq D$. Therefore, since $H_{f^{*}}(X|Z, S)\leq D$, $f^{*}$ is also solution of \eqref{eq: chp5_frl_proof}.


\textbf{case (II)}: Let denote $D^{'}$ the value of the distortion achieved by $g^{*}$. Then, $D^{'}= H_{g^{*}}(X|Z, S) < D$. We have
 \begin{equation}
 \label{eq: id}
\begin{split}
I(D) &= I_{g^{*}}(Z, X) + H_{g^{*}}(X|Z, S) - H(X|S)\\
     & = I_{g^{*}}(Z, X) + D^{'} -H(X|S) \\
     & \overset{(a)} {\geq} R(D^{'}) + D^{'} -H(X|S), \\
     \end{split}
\end{equation}
where $(a)$ follows from the definition of $R(D^{'})$. By convexity of the rate-distortion function, we have that
\begin{equation}
\label{eq: conv}
\begin{split}
R(D^{'}) - R(D) & \overset{(a)}{\geq} \frac{\partial R(D)}{\partial D} (D^{'}- D) \\
&\overset{(b)}{\geq} (D- D^{'}),
\end{split}
\end{equation}
where $(a)$ uses the convexity of $R(D)$ and that $D^{'}<D$ and $(b)$ uses that $\frac{\partial R(D)}{\partial D}\leq -1$. Hence, by combining \eqref{eq: id} and \eqref{eq: conv}, we have
\begin{equation}
I(D) \geq R(D) +D -H(X|S) = I_{f^{*}}(Z, X) + D -H(X|S).
\end{equation}
Therefore, $f^{*}$ is also solution of the minimization \eqref{eq: chp5_frl_proof} since $H_{f^{*}}(X|Z, S)\leq D$. 
\end{proof} 


It  follows from Lemma \ref{lem: 2} that we have by definition of $f^{*}$, if $\frac{\partial R(D)}{\partial D}\leq -1$
\begin{equation}
\label{eq: id_P}
I(D) = I_{f^{*}}(Z, X) + D - H(X|S) = R(D) + D - H(X|S),
\end{equation}
which proves the first part of the statement in Theorem 2.1. Moreoover, if $\frac{\partial R(D)}{\partial D}< -1$, $\frac{\partial I(D)}{\partial D} = \frac{\partial R(D)}{\partial D} + 1 <0$, hence $I(.)$ is decreasing for $D$ such that $\frac{\partial R(D)}{\partial D} < -1$.

To prove that if $\frac{\partial R(D)}{\partial D}\geq -1$, $I(D)=0$, we first prove the following Lemma:
\begin{lem}
Let $D^{*}$ denote the value of $D$ such that $\frac{\partial R(D)}{\partial D}= -1$. For $D^{*}\geq D$, $I(D)=I(D^{*})$. 
\end{lem} 

\begin{proof}
Let $D>D^{*}$. Let $g^{*}$ be a solution of the minimization \eqref{eq: chp5_frl_proof} for $D$. Note that a solution of \eqref{eq: chp5_frl_proof}  for $D^{*}$ respects the constraint of the minimization \eqref{eq: chp5_frl_proof}  for $D$ and thus, $I(D^{*})\geq I(D)$. Let $D^{'}$ denote $H_{g^{*}}(X|Z, S)$. Then, by definition of the rate-distortion objective value \eqref{eq: ib_proof}, we have
\begin{equation}
\begin{split}
I(D) &= I_{g^{*}}(Z, X) + D^{'} - H(X|S) \\
& \geq R(D^{'}) + D^{'} - H(X|S). 
\end{split}
\end{equation}
If $D^{'}< D^{*}$, then we already know that $I(D^{'}) = R(D^{'}) + D^{'} - H(X|S)$ and that $I(D^{'}) > I(D^{*})\geq I(D)$. Moreover, by inequality \eqref{eq: id_P}, $\geq I(D^{'})$, thus $I(D^{'}) > I(D)\geq I(D^{'})$, which is a contradiction. If $D^{'}=D^{*}$, we already know that $I(D)\leq I(D^{*}) = R(D^{*}) +D^{*}-H(X|S)=I(D^{'})\leq I(D)$ and thus that $I(D)=I(D^{*})$. 

It remains to look at the case $D^{'}> D^{*}$. Consider $D^{"}\in [D^{*}, D^{'}]$. By convexity of $R(D)$ we have 
\begin{equation}
\begin{split}
R(D^{*}) - R(D^{'}) &\leq \frac{\partial R(D^{*})}{\partial D} (D^{*} - D^{'})\\
& \overset{(a)}{=} D^{'} - D^{*},
\end{split}
\end{equation}
where $(a)$ comes the fact that $\frac{\partial R(D^{*})}{\partial D}= -1$. It results that by the inequality \eqref{eq: id_P} $I(D)\geq R(D^{*}) + D^{*} -H(X|S)$. Moreover, we already know that $R(D^{*}) + D^{*} -H(X|S)=I(D^{*})$. Hence $I(D^{*})\geq I(D)\geq I(D^{*})$, which proves the equality in Lemma \ref{lem: 2}. 
\end{proof}

\begin{lem}
\label{lem: 3}
Let $D^{**}=H(X|S)$. We have $I(D^{**})=0$.
\end{lem}

\begin{proof}
Consider an encoder $g$ that generates a random variable $Z$ independent of $X$. Then $H_{g}(X|Z, S) = D^{**}$ and $I_{g}(Z, X)=0$. Therefore, $g$ respect the constraint of the minimization \eqref{eq: chp5_frl_proof} for $D^{**}$ and $I(D^{**}) \leq I_{g}(Z, X) + H_{g}(X|Z, S) - H(X|S) = 0$. Hence, $I(D^{**}) = 0$.  
\end{proof}

By combining Lemma \ref{lem: 2} and \ref{lem: 3}, we can show that $I(D)=0$ for $D\geq D^{**}$. 

\section{Lower Bound on $I(Z, S)$}
When constructiong unfairness-distitortion curves, we approximate the mutual information $I(Z,S)$ with an adversarial lower bound. For any approximation $q(s|Z)$ of $p(s|Z)$, we have
\begin{equation}
\label{eq: lb_mutual}
\begin{split}
    I(Z, S)& = H(S) - H(S|Z) \\
    &= H(S) - E_{s,z}[-\log q(s|z)] + KL(p(s|z)||p(s|z) \\
    &\geq H(S) - E_{s,z}[-\log q(s|z)],
    \end{split}
\end{equation}
where the inequality comes from the non-negativity of the Kullback-Leibler divergence $KL(p|q)$. Therefore, we lower bound $I(Z, S)$ with 
\begin{equation}
H(S) - \min_{q}E_{s,z}[-\log q(s|z)],
\end{equation}
where the minimum is taken over classifiers that predict $S$ from $Z$.

\section{Bit Disparity}
In the main test, we make the following claim:
\begin{lem}
\label{lem: 4}
For $\mathcal{S}=\{0, 1\}$, $I(Z, S)\geq g(\pi, \Delta(b))$, where $g$ is an increasing non-negative convex function and $\pi=P(S=1)$. 
\end{lem}

\begin{proof}
The proof is based on a result from ~\cite{gupta2021controllable} applied to a classifier $c_{b}$ that returns $1$ if and only $b=1$: the demographic disparity of $c_{b}$ is exactly $\Delta(b)$ and thus, by Theorem 2.1 in ~\cite{gupta2021controllable}, there exists a non-negative, convex and increasing function $g$ such that 
\begin{equation}
    I(Z, S) \geq g(\pi, \Delta(b)).
\end{equation}
\end{proof}
